From Questions to Insightful Answers: Building an Informed Chatbot for University Resources

This paper presents BARKPLUG V.2, a Large Language Model (LLM)-based chatbot system built using Retrieval Augmented Generation (RAG) pipelines to enhance the user experience and access to information within academic settings.The objective of BARKPLUG V.2 is to provide information to users about various campus resources, including academic departments, programs, campus facilities, and student resources at a university setting in an interactive fashion. Our system leverages university data as an external data corpus and ingests it into our RAG pipelines for domain-specific question-answering tasks. We evaluate the effectiveness of our system in generating accurate and pertinent responses for Mississippi State University, as a case study, using quantitative measures, employing frameworks such as Retrieval Augmented Generation Assessment(RAGAS). Furthermore, we evaluate the usability of this system via subjective satisfaction surveys using the System Usability Scale (SUS). Our system demonstrates impressive quantitative performance, with a mean RAGAS score of 0.96, and experience, as validated by usability assessments.

==> completions_table.tex <==
\begin{table}[ht]
{\renewcommand{\arraystretch}{1.30}%

\begin{tabular}{p{4cm}|p{4.0cm}}

\hline
%\rowcolor{cyan!20!}
\textbf{Prompt}  & \textbf{Completion} \\ \hline

Who do I contact if I have additional questions about majors or   attending MSU?   & Graduate   students in the Computer Science and Engineering (CSE) department at   Mississippi State University have access to a range of funding opportunities   to support their academic pursuits. These include graduate assistantships,   research grants, fellowships, scholarships, and industry partnerships.   Graduate assistantships offer stipends and tuition waivers in exchange for   research or teaching assistance, while research grants cover project   expenses. \\ \hline

What are the funding opportunities available for graduate   students in the CSE department? &For queries on majors and admissions at Mississippi State   University, reach out to the Office of Admissions and Scholarships at   662-325-2224 or admissions@msstate.edu. For academic guidance, contact   departmental advisors or the Career Center at 662-325-3344 or   career@career.msstate.edu for current students, aiding with course   requirements, career prospects, and internships. \\ \hline




                                    
\end{tabular}}
\\
\\
\caption{Completions}

\label{table:dt_intro}
\vspace{-2mm}

\end{table}

==> old_content.tex <==
% \subash{this is incorrect...acquire knowledge??}. 
% within the evolving landscape of course structures and curriculum demands, Machine Learning (ML), and Large Language Models (LLMs) emerge as essential pillars, enabling the delivery of a tailored and enriching learning experience 
%\hl{this whole paragraph is so disconnected ...its does not reflect what you are trying to paint here??}.

% As new student-led clubs, events, dates, and resources are announced, navigating through various web pages and university online platforms becomes increasingly time-consuming to locate the necessary information. Exploring and scouring and multiple webpages to find relevant information can become cumbersome and not accessible for everyone. What is needed is a service that can process all the university resources to provide more intelligent analysis of the university-related contents and respond interactively providing the ground for easier access to relevant information.
% \subash{again, we want to be consistent with 1 idea and stick with it..is it HCI that we want to improve? Is is peronalized CHATBOT?} 
%\hl{rephrase the above sentence it reads and seems convulated}



% Given the ongoing research and interest in Artificial Intelligence (AI), Machine Learning (ML), and Large Language Models (LLMs), there exists foundational development for advanced technologies to improve personalized human-computer interactions fostering a dynamic, user-driven experience. LLMs, such as Chat-GPT, Llama, and Gemini, leverage powerful inference capabilities to analyze large bodies of data. However, they often perform poorly on data outside their training dataset, leading to hallucinated generated outputs. One innovative approach to address this challenge is Retrieval-Augmented Generation (RAG) pipelines \cite{lewis2021retrievalaugmented}. RAG integrates the strengths of both knowledge retrieval and generation models, enabling LLMs to ingest retrieved evidence and contextual information from external sources before generating responses. This process empowers LLMs to provide more accurate and informed answers, enhancing their performance across diverse datasets and domains.

% Given the ongoing research and interest in Artificial Intelligence (AI), Machine Learning (ML), and Large Language Models (LLMs), there exits foundational development for advanced technologies to imporve personalized human-computer interactions fostering a dynamic, user-driven experience. 
% % \subash{what does this first sentence mean??} 
% LLMs in particular are known for their powerful inference capabilities in analyzing large body of data. Some LLMs models such as Chat-GPT, Llama, and Gemini are examples of AI systems that can provide responsive instructions following the prompts 
% % \subash{may be we should not be assertive as it may not not provide ``Optimal response" also...start using words such as ``instruction following", ``prompt", "completions" etc}
% from the contents they have been trained on.
% % \subash{don't use data}
% However, they perform poorly on data outside their training dataset, which can result in hallucinated generated outputs. 
% % \subash{I get the picture but this sentence need a rephrase.}. 
% One way to address this problem, Retrieval-Augmented Generation (RAG) \cite{lewis2021retrievalaugmented}
% % \subash{cite this} 
% pipelines have been developed 
% % \subash{Also, RAG is one possible way to "mitigate" hallucination..there are other approach as well..eg. ``Finetuning"}. 
% With RAG pipeline LLMs can read through the new data and then create inferences on the new data and provide reasonable answers. 


% \subash{you need to write 2-3 sentence about RAG before you jump to conclusion abot what RAG does...while doing so use words such as ``Knowledge Ingestion" ..``retrieved evidence", ``context" etc with an example.}\

% \elias{I have modified that part. Its completed}

% From the academic perspective, in today's rapidly changing educational scene, Mississippi State University (MSU) has the challenge of making its growing resources easily available and in a user-friendly fashion. To address this, we have released \AlgoName, an AI-powered chatbot created at the Predictive Analytics and Technology Integration Laboratory (PATENT) Lab at MSU. This application is specifically developed to improve students and staff engagement with university resources.

% \AlgoName distinguishes itself by providing rapid, 24x7 access to a wide range of information, including academic program specifics, policies and campus event announcements. It is designed on the Django framework, which allows users to engage with a simple login, making it both secure and user-friendly. The chatbot accesses massive amounts of data from over 42 departments,
% % {please double check this}
% providing not just responses but also individualized insights based on the most recent AI and machine learning technology.


\begin{comment}
    



\IEEEPARstart{E}{FFE}ctive communication is essential for colleges and universities to convert potential applicants into enrolled students. When admission processes are prolonged, prospective students often seek assistance on university websites. However, delayed responses can deter students, particularly during high application periods, leading to negative reviews and decreased interest, ultimately impacting university revenue.

Amidst these challenges, advancements in technology have introduced transformative solutions to enhance communication channels. Generative AI, as a subset of artificial intelligence, has emerged as a significant force in revolutionizing how universities engage with their prospective and current students. This technology has facilitated the development of modern chatbot applications such as OpenAI’s ChatGPT \cite{openai2024gpt4}, Microsoft Bing \cite{dao2023evaluation}, and Google Gemini \cite{geminiteam2024gemini} . However, the inherent limitations of generative AI, particularly through LLMs, have posed challenges, including the poor performance of LLMs when encountering data outside their training dataset. 

Nevertheless, innovative approaches such as Retrieval-Augmented Generation (RAG) pipelines have emerged to address these constraints. RAG integrates the strengths of both knowledge retrieval and generation models, allowing LLMs to ingest contextual information and evidence from external sources before generating responses. By leveraging this approach, LLMs can provide more accurate and informed answers, enhancing their performance across diverse datasets and domains.


From the academic perspective, Mississippi State University (MSU) grapples with the task of ensuring its expanding resources are readily accessible and user-friendly. This challenge is where the potential of generative AI, particularly in chatbot applications, becomes evident. To address this need, \AlgoName was developed at the Predictive Analytics and Technology Integration Laboratory (PATENT) Lab at MSU. This AI-powered chatbot is specifically designed to improve accessibility to university resources, offering rapid, 24x7 access to a wide range of information, including academic program specifics, policies, and campus event announcements. By leveraging the latest AI and machine learning technology, \AlgoName not only offers immediate responses but also delivers personalized insights tailored to the unique needs of each user. This personalized approach enhances engagement and improves the overall user experience throughout the university community. 

% AI-based technologies such as OpenAI's Chat-GPT\cite{openai2024gpt4}, Llama\cite{touvron2023llama}, and Gemini\cite{geminiteam2024gemini} exemplify the cutting-edge capabilities of artificial intelligence in simulating interactive environments for users to seamlessly accessing and processing educational content and benefit from personalized support
\end{comment}




% This part of the qualitative assessment focuses on particular interactions between prospective and current students and the affiliated faculty members. The figures presented demonstrate different types of inquiries made by users and the corresponding responses provided by the BarkPlug v.2. By capturing these interactions and analyzing them, the research aims to evaluate BarkPlug v.2's ability to comprehend and respond to user queries. Figure \ref{fig:initial_inquiry} portrays the system's response to an initial inquiry from a prospective student, demonstrating its capacity to engage users by offering relevant information from the outset. Figure \ref{fig:live_interaction} highlights the system's ability to handle real-time questions and maintain a conversational flow during a live interaction with a current student. Figure \ref{fig:detailed_question} offers insights into BarkPlug v.2's performance when presented with a detailed and specific question from a faculty member, assessing its capacity while experiencing complex queries.
% Figure \ref{fig:follow_up_query} examines the chatbot's handling of a follow-up query from a prospective student, showcasing its ability to manage ongoing conversations and provide comprehensive answers that build on previous interactions.


%evaluated the efficacy of our BarkPlug v.2 using the System Usability Scale (SUS) \cite{vlachogianni2022perceived}. This widely recognized and reliable method swiftly assesses system usability through a set of ten questions, each offering five response options ranging from “strongly agree” to “strongly disagree”.


%Qualitative – users’ stress responses (facial reactions, body-language changes, squinting, etc.), subjective satisfaction (which they give through a post-test questionnaire) and perceived level of effort/difficulty

% \st{"}\hl{``}strongly agree" to "strongly disagree", as elaborated in Table \ref{tab:sus_questionnaire} of Appendix~\ref{app:sus_table} \hl{reference mismatch}. \subash{update opening double quotes as highlighted above} %Following our use of the SUS to assess the usability of BarkPlug v.2, we collected detailed feedback from participants of the Seminar (CSE8011) course at Mississippi State University. A total of 50 individuals evaluated the system's performance. 

%This is to say that a score below 68 suggests significant usability concerns necessitating attention, while a score exceeding 68 denotes satisfactory usability \cite{kaya2019usability}. Furthermore, scores of 80.3 or higher are classified as an A, reflecting excellent user satisfaction, while scores around 68 represent a C, indicating average usefulness with room for improvement. Given our SUS score of 68.41\%, it is evident that this system is practical for real-world application within the university setting. In addition to the SUS assessment, Fig. \ref{fig:bar-sus}. presents the comprehensive responses of the participants, identifying specific areas for improvement within the BarkPlug v.2 system through visual representation.



%We proceeded by employing the RAGAS framework and establishing a vector database using the embeddings extracted from the master JSON file (detailed in Section \ref{implementation-detail}).To assess the retriever's efficacy, we employed two distinct methodologies: an Ensemble Retriever and one rooted in the Chroma Database. The Chroma Database retriever employs similarity thresholds and maximum marginal relevance (MMR) search methods. Since RAGAS assesses the RAG pipeline based on four distinct metrics such as context precision, context recall, faithfulness, and answer relevance, therefore, we presented the mean score for each category in Table \ref{tab:different_retrieval_scores}. In our evaluation, the answer relevance score of RAGAS (mean score) ranged from 0.89 to 0.99 on a scale from 0 to 1, with 1 representing optimal generation.



% In this section, the distributions and correlations of a variety of contextual question-answering performance-related evaluation metrics are examined. The histograms depicted in Figure \ref{fig:distribution_plot} illustrate the distinct outcomes of four metrics, namely Context Precision, Context Recall, Faithfulness, and Answer Relevancy \cite{keswani2024abstractive}. Although certain data points contain extraneous information, Context Precision scores are generally high, indicating that the contexts are generally pertinent. The bimodal nature of context recall indicates that there is some variation in the extent to which contexts adequately convey the essential information, as evidenced by the fluctuations between high and low recall. A high grade for faithfulness generally indicates that the responses provided are accurate in general; however, intermittently lesser grades may indicate the presence of certain inaccuracies. The responses are largely pertinent to the questions, as evidenced by the high relevance of the answers.


% Figure \ref{fig:heatmap_plot}, also known as the Correlation Heatmap \cite{buyrukouglu2022machine}, vividly displays the relationships among different evaluation metrics. The heatmap shows a strong positive correlation between context recall and faithfulness (r = 0.8), highlighting that as more relevant information from the context is included, the answers tend to more accurately reflect this context. Correlations between other metrics are generally moderate to low, indicating that precision and relevancy largely operate independently from each other and from recall and faithfulness.

\vspace{0.1cm} % Add space here

% One the other hand, Table \ref{tab:summary_stats} \subash{merge these tables} present summary statistics for each metric, quantifying the observations made in this study. Average scores for context accuracy and reliability are particularly high, highlighting the system's strong performance in providing relevant context and correct answers. Consistently high average scores across all metrics, including context recall and answer relevance, demonstrate the system's effectiveness in capturing essential information and remaining relevant to the questions asked. The ranges indicated by the minimum and maximum values show the system's ability to achieve perfect scores under various conditions, reflecting its ability to consistently provide accurate and reliable feedback.

% One the other hand, Table \ref{tab:summary_stats} present summary statistics for each metric, quantifying the observations made in this study. Average scores for context accuracy and reliability are particularly high, highlighting the system's strong performance in providing relevant context and correct answers. Consistently high average scores across all metrics, including context recall and answer relevance, demonstrate the system's effectiveness in capturing essential information and remaining relevant to the questions asked. The ranges indicated by the minimum and maximum values show the system's ability to achieve perfect scores under various conditions, reflecting its ability to consistently provide accurate and reliable feedback.

\vspace{0.1cm} % Add space here

% In addition, Table \ref{tab:question_categories} depicts the average assessment scores for different categories of questions. This proves that the "engineering program" has high precision, reliability, and relevance, although its recall is somewhat low. "General Investigation" achieves perfect scores in recall and fidelity. "Scope of research" shows great precision and recall, but faces difficulties with fidelity and relevance. “University Resources” performs well in precision and recall, yet struggles to deliver precise and relevant responses concerning university resources.


% For the first image
% \begin{figure*}[ht!]
% \centering
% \includegraphics[width=0.6\textwidth, height=0.35\textheight]{larger_label_high_res_distribution_plots.png} 
% \caption{Distribution plots of context precision, context recall, faithfulness, and answer relevancy.}
% \label{fig:distribution_plot}
% \end{figure*}

% For the second image
% \begin{figure*}[ht!]
% \centering
% \includegraphics[width=0.6\textwidth, height=0.35\textheight]{heatmap_smaller_values.png} % Adjust the width and height as needed
% \caption{Statistical relationships between context precision, context recall, faithfulness, and answer relevancy.}
% \label{fig:heatmap_plot}
% \end{figure*}

% \begin{table}[ht!]
% \centering
% \caption{Summary statistics for the evaluation scores.}
% \label{tab:summary_stats}
% \begin{tabular}{lcccc}
% \toprule
% Metric            & Mean  & Std Dev & Min & Max \\
% \midrule
% Context Precision & 0.962 & 0.099   & 0.500 & 1.000 \\
% Context Recall    & 0.929 & 0.220   & 0.000 & 1.000 \\
% Faithfulness      & 0.982 & 0.055   & 0.750 & 1.000 \\
% Answer Relevancy  & 0.945 & 0.159   & 0.000 & 1.000 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % For the left-side table
% \begin{table}[ht!]
% \centering
% \caption{Summary statistics for the evaluation scores.\hl{Merge table 1 and 2}.}
% \label{tab:summary_stats_left}
% \begin{tabular}{lcccc}
% \toprule
% Metric            & Mean  & Std Dev & Min & Max \\
% \midrule
% Context Precision & 0.962 & 0.099   & 0.500 & 1.000 \\
% Context Recall    & 0.929 & 0.220   & 0.000 & 1.000 \\
% \bottomrule
% \end{tabular}
% \end{table}

% % For the right-side table
% \begin{table}[ht!]
% \centering
% \caption{Summary statistics for the evaluation scores (continued) \hl{Merge table 1 and 2}.}
% \label{tab:summary_stats_right}
% \begin{tabular}{lcccc}
% \toprule
% Metric            & Mean  & Std Dev & Min & Max \\
% \midrule
% Faithfulness      & 0.982 & 0.055   & 0.750 & 1.000 \\
% Answer Relevancy  & 0.945 & 0.159   & 0.000 & 1.000 \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table*}[ht!]
% \setlength{\tabcolsep}{4pt} % Adjust the horizontal spacing between columns
% \centering
% \caption{Average Evaluation Scores by Question Category}
% \label{tab:question_categories}
% \begin{tabular}{l*{4}{>{\centering\arraybackslash}p{1.5cm}}}
% \hline
% \textbf{Category} & \rotatebox{90}{\textbf{Ctx. Prec.}} & \rotatebox{90}{\textbf{Ctx. Recall}} & \rotatebox{90}{\textbf{Faith.}} & \rotatebox{90}{\textbf{Ans. Rel.}} \\
% \hline
% Engineering Programs & 0.963 & 0.899 & 0.986 & 0.978 \\
% General Inquiry & 0.958 & 1.000 & 1.000 & 0.983 \\
% Research Opportunities & 0.944 & 1.000 & 0.958 & 0.917 \\
% University Resources & 0.967 & 1.000 & 0.958 & 0.747 \\
% \hline
% \end{tabular}
% \end{table*}

% \subsubsection{Comparative Analysis of Retrieval Efficiency}
% \label{app: retrieval-efficiency}

% \subash{This should be evident in Section 3..You need to explain that you have multiple retrieving techniques}
% This section explains the various retriever outcomes that were employed to assess the performance of our LLM. These outcomes include the \emph{maximum marginal relevance retrieval (MMR), similarity score threshold retrieval}, and \emph{ensemble retriever}. \subash{Start italicizing the important words within the text as seen in the sentence above} Table \ref{tab:different_retrieval_scores} shows the average assessment scores based on questions category and three different retrievals. Table \ref{tab:different_retrieval_scores} evaluates each retrieval on four academic areas, based on context precision, context recall, faithfulness, and answer relevancy. It is to be mentioned that all approaches receive good ratings, indicating their overall efficacy. To further emphasize, \st{s}\hl{S}imilarity Threshold Retrieval excels at accurately matching the specific purpose of queries, as evidenced by its high precision and faithfulness scores. Furthermore, \hl{MMR} \subash{acronym not defined earlier in the text} Retrieval maintains its high results, despite a modest drop in precision within the Engineering Programs. In addition to these, Ensemble Retrieval stands out with unusually high recall values, particularly in the Research Opportunities and University Resources categories, implying that it is considerably incredible at discovering relevant information. 

% Figure \ref{fig:heatmap_plot_overall} also evaluates three retrieval strategies. It demonstrates the effectiveness of all techniques, with the Similarity Threshold method excelling in precision and faithfulness, and the Ensemble method attaining exceptional recall, particularly in General Inquiry and University Resources. The MMR technique demonstrates balanced performance in all categories.


% \begin{table*}[ht!]
% \centering
% \caption{Average Evaluation Scores by Question Category and Retrieval Type}
% \label{tab:different_retrieval_scores}
% \begin{tabular}{@{}lcccccccccccc@{}}
% \toprule
% & \multicolumn{4}{c}{Similarity Threshold} & \multicolumn{4}{c}{MMR} & \multicolumn{4}{c}{Ensemble Retrieval} \\
% \cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13}
% Category & \multicolumn{1}{l}{Prec.} & \multicolumn{1}{l}{Recall} & \multicolumn{1}{l}{Faith.} & \multicolumn{1}{l}{Rel.} & \multicolumn{1}{l}{Prec.} & \multicolumn{1}{l}{Recall} & \multicolumn{1}{l}{Faith.} & \multicolumn{1}{l}{Rel.} & \multicolumn{1}{l}{Prec.} & \multicolumn{1}{l}{Recall} & \multicolumn{1}{l}{Faith.} & \multicolumn{1}{l}{Rel.} \\
% \midrule
% Engineering Programs & 0.98 & 0.96 & 0.99 & 0.97 & 0.95 & 0.97 & 0.98 & 0.96 & 0.97 & 0.98 & 0.98 & 0.97 \\
% General Inquiry & 0.95 & 0.97 & 0.98 & 0.96 & 0.97 & 0.98 & 0.98 & 0.96 & 0.96 & 0.99 & 1.00 & 0.945 \\
% Research Opportunities & 0.97 & 0.98 & 0.96 & 0.99 & 0.97 & 0.98 & 0.96 & 0.97 & 0.96 & 0.98 & 1.00 & 0.945 \\
% University Resources & 0.96 & 0.99 & 0.97 & 0.98 & 0.97 & 0.98 & 0.97 & 0.98 & 0.96 & 0.99 & 0.86 & 0.89 \\
% \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table*}[ht!]
% \centering
% \caption{Average Evaluation Scores by Question Category and Retrieval Type}
% \label{tab:different_retrieval_scores}
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% & \multicolumn{4}{c}{Similarity Threshold} \\
% \cmidrule(r){2-5}
% Category & \multicolumn{1}{l}{Prec.} & \multicolumn{1}{l}{Recall} & \multicolumn{1}{l}{Faith.} & \multicolumn{1}{l}{Rel.} \\
% \midrule
% Engineering Programs & 0.98 & 0.96 & 0.99 & 0.97 \\
% General Inquiry & 0.95 & 0.97 & 0.98 & 0.96 \\
% Research Opportunities & 0.97 & 0.98 & 0.96 & 0.99 \\
% University Resources & 0.96 & 0.99 & 0.97 & 0.98 \\
% \bottomrule
% \end{tabular}
% \end{table*}

%% %to examine how well our system performs specifically designed for assessing Retrieval-Augmented Generation (RAG) pipelines. due to the unsuitability of other commonly used metrics, such as ROUGE \cite{lin2004rouge} and BLEU \cite{papineni2002bleu}. BLEU is mostly used for machine translation task evaluation, whereas ROUGE is intended for text summarization task evaluation. %These metrics prioritize comparing the structure of generated sentences to the reference ones, which is not suitable for our case where sentences might have different structures but convey the same information accurately. %In our evaluation process, we initially established ground truths across eight engineering departments at Mississippi State University. 


%Subsequently, using the LangChain library's RecursiveCharacterTextSplitter \cite{topsakal2023creating}, we split text and created embeddings with OpenAI's text-embedding-3-large model \cite{harris2024enhancing}, storing them in Chroma Database. This database allowed us to retrieve documents relevant to specific queries using a similarity threshold search method. These documents, along with their queries, were processed through OpenAI's GPT-3.5 Turbo models \cite{rasheed2024large}.


%For the system integration phase, we leveraged Django \cite{dauzon2016django}, a versatile Python framework, to handle both the front-end and back-end management. This setup included user authentication features and an interactive chatbot interface to enhance user engagement. 

%Initially, the chatbot only supports the English language, which restricts accessibility for non-English speaking users. Moreover, it lacks capabilities such as Automatic Speech Recognition (ASR) and text conversion, confining user interactions to typing.Furthermore, its information retrieval system sometimes fails to provide accurate or relevant results, occasionally producing incorrect information known as `hallucinations.' Additionally, a significant limitation is the 16385 token limitation of the OpenAI API, which restricts the length of interactions our chatbot can process at one time.



% chatbot application development in educational settings.

% \subash{Remove ``subsubsection" and include a phrase like highlighted below. Rephrase in your own words.}
% \hl{In this section, we briefly look into the pre-requisite background and related developments in the context chatbot application development in educational settings.}



%\subsection{Background}
% \subsection{Large Language Models (LLMs)}
% In recent years, Large Language Models (LLMs) have been utilized across various sectors, including cybersecurity, law, and education, owing to their capacity to generate human-like responses 
% % \subash{may be human-like ``response" is better}
% and their utility in addressing linguistic challenges. Particularly within the education sector, LLMs are employed to provide assistance and support to learners \cite{latif2023knowledge}. LLMs are built upon the original Transformer model (seq2seq) \cite{vaswani2023attention} and are engineered to undertake a wide array of Natural Language Processing (NLP) tasks, such as summarization and question answering. These models undergo training on extensive datasets encompassing diverse topics from various sources such as publicly available contents on internet, books, licensed third parties.  
% % \subash{I believe it is massive internet crawls and publicly avaliable...at least what they say..please double check} . 
% Their capabilities expand alongside the growth of their trained parameters. However, a drawback of pre-trained LLMs is their tendency to ``hallucinate" when presented with unseeded data. Hallucination refers to the phenomenon where LLMs generate responses that fail to address the query at hand, resulting in irrelevant outputs \cite{zhang2023siren}. 


% \subsection{Retrieval Augmented Generation (RAG)}
% % \hl{start with drawback of PLMs and showcase Rag's potential in alleviating stated problems with PLMs}

% LLMs may struggle with domain adaptation and magnify biases, producing outputs that are irrelevant or erroneous. These problems can be made worse by sparse or skewed fine-tuning data, which can lead to delusional replies that are not coherent or broadly applicable. As the demand for alleviating hallucination problem with LLMs increases, models such as Retrieval-Augmented Generation (RAG) \cite{lewis2021retrievalaugmented} have been proposed to combat model hallucination and provide a cost-effective solution for feeding the model new knowledge to work with \cite{wu2024faithful}. This approach avoids the need for fine-tuning the parameters, which can be computationally costly, especially when dealing with billions of parameters. 
% \subash{if possible cite this statement}. 
% Through the use of RAG, the Generative AI system can access more information beyond their training parameters to generate more robust and domain specific content.
% \subash{this sentence does not make sense}.
% By doing so, it offers a hybrid solution that reduces hallucinatory answers and produces more factual responses. \subash{give some example how RAG actually works?? }\cite{ma2024megalodon} \cite{wu2024reliable}

% \subsection{Related Work}
% Given the progress achieved in the development of question-answering systems for a wide range of purposes, including university admission procedures, it is imperative to critically assess current methodologies and their constraints in order to pinpoint potential avenues for additional investigation and advancement.
% \subash{related work is too long..it provides the summary of others work but doesnot compare with our own system...please trim and if possible find their limitation and explain if our approach/application is better than theirs in that regard.}

% In \cite{chandra2019indonesian}, Yogi Wisesa Chandra et al. developed a question-answering system tailored for university admission in Indonesia using a Sequence-to-sequence learning (Seq2Seq) model. %They showcased the effectiveness of the Seq2Seq approach coupled with attention mechanisms in crafting context-aware question and answering systems. The models they constructed utilized a two-layered LSTM as both encoder and decoder, and they employed data augmentation techniques to alleviate the constraints posed by limited training data. Their experimentation comprised two main phases: evaluation and testing. In the evaluation phase, they opted not to integrate the attention mechanism, resulting in a Bilingual Evaluation Understudy (BLEU) score of 43.61\%. However, in the testing phase, the inclusion of the attention mechanism led to a notable improvement, with the BLEU score rising to 44.68\%. Despite these outcomes, the study did not address challenges related to out-of-vocabulary issues, nor did it provide insights into how contextual relevance of answers was ensured.

% Expanding on the advancements in question-answering systems, Oliveira et al. \cite{oliveira2023introducing} ventured into enhancing student interaction with their creation of a chatbot. This chatbot could have dynamic conversations with students on a wide range of topics. It could help with admissions, finding study materials, understanding course requirements, picking courses, accessing academic support, using campus services, joining clubs, learning about events, and scheduling appointments. What made this chatbot remarkable was how it focused on students' needs. Oliveira and the team listened to feedback from students, teachers, and staff to make sure the chatbot worked well for everyone. They also ensured that it was accurate, reliable, and safe through careful testing. Despite its usefulness, it is found that it needed constant updates from websites and documents to stay useful. This shows that even with advanced technology, there is still a need for ongoing improvement to keep up with changes.

% In this manuscript \cite{martinez2024designing}, TutorBot+ is presented as a chatBot developed by Universidad Católica de la Santísima Concepción to offer feedback to students enrolled in programming courses. By emphasizing academic integrity and harnessing Large Linguistic Models (LLMs) such as chatGPT, TutorBot+ aims to enhance the learning experience. The study progresses through four distinct phases: implementation, literature review, experimental design, and instrument development. Throughout the study, each phase is intricately connected, with the literature review informing the development of TutorBot+, which in turn shapes the experimental design. A quasi-experimental study is currently underway to gather data on the tool's impact on students' computational reasoning abilities. Initial findings suggest the viability and potential of TutorBot+ to improve academic achievements. Early feedback from students indicates increased performance and engagement. However, for a comprehensive assessment of its long-term efficacy and implications for academic integrity, further research is necessary.


% In this study \cite{bratic2024centralized}, a composite model that combines an API intended for a large language model (LLM)/chatbot with the transformer framework is introduced. The model ensures accurate responses from a large database of instructional resources by combining these components. The model architecture makes use of mathematically specified methods to enable deep text processing through sophisticated word embedding techniques. This improves natural language comprehension accuracy while preserving high levels of speed and flexibility. This research is important in ways that go beyond just offering a technological solution for a widespread issue. It also emphasizes how new technology can be integrated into education and continue to advance. The ultimate objective is to develop a more efficient, open, and inclusive learning environment that meets the various demands of students all around the world. Furthermore, when communicating with diverse languages through the model's API, it is imperative to recognize the potential issues that may occur in managing linguistic nuances and cultural variances. However, while adding scholarly articles to the model may improve its content, adding relevant data directly to the database could improve the model's functionality and applicability in learning environments.

% This article \cite{kim2023chatgpt} demonstrates the future application of large language models like ChatGPT in academic medicine, based on a scoping review of their current state. Among 87 documents identified through a Medline search, 33 were relevant to LLM ChatBots or ChatGPT, informing the development of five guideline statements. These prioritize human verification, accountability, and transparency in the use of ChatGPT/LLMs. Kim et al. \cite{kim2023chatgpt} are urged to uphold ethical principles when integrating these models into scholarly publications, considering their impact on the healthcare sector. The review underscores the importance of human governance and accountability in leveraging AI technologies in academia, emphasizing the need for careful utilization to maintain research integrity. The guidelines provide a valuable framework for researchers navigating the complex landscape of LLM usage, promoting transparency and accountability in AI-driven research endeavors.


% The objective of the research \cite{vanichvasin2021chatbot} was to construct, assess, and investigate the effects of a chatbot on the research knowledge of university students in Thailand. The research tools comprised the chatbot, evaluation forms, questionnaires, and research exams, and were utilized with the participation of 36 students. It is found that Mean, standard deviation, content analysis, and a t-test were utilized in the analysis. In contrast to the specialists' assessment of the chatbot's high applicability, the students' evaluation of its efficacy recommended the incorporation of additional interactivity and content. Students thought the chatbot was novel and user-friendly; however, they recommended incorporating visual aids such as examples and illustrations to increase engagement. Furthermore, the substantial increase in post-test scores relative to pre-test scores suggests that the students made progress in their learning. As a result of providing a personalized learning environment, the incorporation of chatbot technology into education has had a positive impact on students' research knowledge.

% \vspace{0.1cm} % Add space here

% Even though these studies have shown promising results, there are still issues and problems that need to be resolved. While chatbots have proven useful in offering immediate support and customized learning experiences, problems including out-of-vocabulary, content relevance, and frequent updates are still causes for concern. Furthermore, concerns about accountability, transparency, and ethical issues are brought up by the use of large language models like ChatGPT in educational settings. In order to overcome these obstacles and fully utilize chatbot technology's promise to enhance student learning and academic achievement, more research is required to determine how best to integrate it into the classroom.


% Integrating chatbots into educational settings, especially within university platforms and metaverses, offers promising avenues for improving user experience and facilitating learning. Xie et al. \cite{xie2023chatbot} demonstrate how chatbots in metaverse-based university platforms offer instant, personalized support for tasks like course navigation and FAQs, leveraging NLP and machine learning to streamline information dissemination and reduce administrative burdens. In specific university contexts, Chandra et al. \cite{chandra2019indonesian} develop a question-answering system for Indonesian university admissions using Sequence-to-sequence learning. Similarly, Oliveira et al. \cite{oliveira2023introducing} introduce a dynamic chatbot enhancing student interaction, covering admissions, academic assistance, and event information, prioritizing user feedback for accuracy, reliability, and safety with frequent updates to maintain relevance.

% Martinez et al. \cite{martinez2024designing} present TutorBot+, employing LLMs like ChatGPT to offer feedback in programming courses, showing positive impacts on students' computational reasoning abilities in ongoing quasi-experimental research, illustrating the potential of such interventions in education.



% \subash{Introduce your architecture in few lines..then discuss phases in couple of lines...after that for example begin with something like``This section describes the architecture of \AlgoName...". State you have ``X" tired/phase architecture. Provide brief information about them and include phrases such as ``....the rest of this section describes each phase in detail
% and elaborates on our techniques" at the end.}

% \hl{basically you have 2 phase architecture 1. Retriever 2. Generator, I don't understand why evaluation is attached with architecture? Remove it from Fig 1. }




%Our implementation utilizes a Chroma Database-based retriever with a similarity threshold search method, where the query is compared against stored documents, retrieving those meeting or surpassing a specified similarity threshold. We employed the text-embedding-3-large model for text embeddings due to its superior performance among various OpenAI embedding options. This model converts textual inputs into vector representations to further efficient comparison and retrieval.

%In the second phase, the retrieved evidence plays a vital role where completions are generated using Pre-trained Language Models (PLMs). By leveraging the maximum benefits from openAI's token limit, we provide comprehensive context for PLMs to generate extensive completion, mitigating the risk of “hallucination”. 



%While in the second example the user is seeking information about admission to Mississippi State University. To answer this the system must have knowledge about campus resources such as admission and scholarships. As stated before \AlgoName not only have knowledge about academic department but also other campus resources and one of them is admission and scholarships. Using the admission and scholarships as external data source the relevant document that reflects information about addmission and scholorships along with contact details as seen in Fig \ref{box_final_Completions} is returned as completion to the user. 




%\input{completions_table}

%During the Completion or Response Generation phase, our architectural design integrates effortlessly with the OpenAI GPT-3.5 Turbo API to streamline the response generation process. The initiation of this procedure involves providing the API with the N highest-ranked documents acquired in the previous retrieval phase, in addition to a customized prompt, query, and a set of prompt engineering instructions that ensure the completions produced comply with predetermined limitations. To adhere to the API-mandated token limit of 16k tokens, we implement optimization techniques such as preprocessing and custom chunk size. By organizing the input data, the generated completions can strike a balance between comprehensiveness and conciseness. By integrating the retrieved documents, custom prompt, query, and adherence instructions, we equip the GPT-3.5 Turbo API with rich contextual information, enabling it to produce coherent and informative responses within the defined boundaries

%Additionally, the architecture is made to be efficient and scalable, able to manage high query volumes and provide timely, high-quality results. As the cornerstone of our RAG system, the Completions or Response Generation phase ensures the delivery of contextually appropriate and high-quality responses to user requests while adhering to set limitations.



% \hl{Describe you contextualize the retrieved evidence and perform completions here}


% \textbf{Preprocessing}
% \subash{this stuff about data should go into results section and should have a small subsection with heading such as ``Dataset" where you describe your dataset and your approach to curate and pre-process the data.}

% We develop a crawler to gather unbiased and diverse information from all MSU architecture departments. This process yields 42 JSON files,
% % \subash{in introduction you said 100 departments, here you are suggesting 42? Can we be consistent?}
% which are then consolidated into a master JSON file. Subsequently, we denoise the master JSON to remove unwanted Unicode characters.

% Our primary goal is efficient document retrieval and keyword extraction. To achieve this, we implement a multi-step process:

% \begin{enumerate}
%     \item \textbf{Document Segmentation}: We employ a recursive text splitter to divide research papers into chunks. Parameters such as chunk size and overlap dictate the segmentation strategy.
%     \item \textbf{Text Embedding}: Using an embedding model, we convert text data into vector representations. This model can be chosen from existing options or customized to suit our needs.
%     \item \textbf{Local Repository}: The vectorized data is stored locally, forming our repository of architectural research knowledge.
 
% \end{enumerate}

% Gathering all our well-organized data into a single database makes our model's work much smoother. Instead of rummaging through separate databases for each department, it finds what it needs in one place. This speeds up our responses and saves time. Moreover, by eliminating noise and inconsistencies, the LLM can better understand and utilize the information available, resulting in higher-quality outputs.


% \textbf{Architecture}

% Upon receiving a user query, our system initiates by retrieving the top-n documents, with 'n' representing a predetermined value. Subsequently, our Language Model (LLM), which may include options like Mistral or LLAMA2, processes this data and generates responses, ensuring the continuity of our Retrieval-Augmented Generation (RAG) system. Post-RAG execution, the test phase involves submitting queries, responses, context, and ground truth for evaluation. Ragas, a robust library, facilitates RAG pipeline assessment by capturing input/output/context triplets and deriving metrics across various pipeline components. Evaluation encompasses four key metrics: Faithfulness, Answer Relevancy, Context Precision, and Context Recall, with a focus on Retrieval and Generation modules. Retrieval metrics assess context relevance and recall, while Generation metrics evaluate answer pertinence and factual consistency. Through Ragas, we measure the correctness and coherence of our answers.

% \subash{We need to work more in this section as it's the core of the paper..right now it's super weak...}


\begin{comment}
\subsection{Preprocessing}


In the pre-processing step, we begin by acquiring JSON files containing meticulously cleaned and extracted data relevant to our specific use case. Our primary objective is to efficiently manage the retrieval of documents, necessitating the extraction of keywords and their respective frequencies. 

To achieve this, we employ a multi-step process. Initially, we load the documents and apply a recursive text splitter, dividing the text into chunks. These chunks are defined by parameters such as chunk size which determines the length of each segment, and chunk overlap to dictate the degree of overlap between consecutive segments.

Following the segmentation of documents, we utilize an embedding model to convert the text data into vector representations. This embedding model can be selected from existing options or customized according to our requirements. Once the transformation into vector data is complete, we archive it on our local machine, constituting our repository of local knowledge.

\begin{figure}[h]
\centering
    \includegraphics[scale=0.25]{figs/Embeddings_Arch.png}
    \caption{Converting documents to vector DB. \hl{update this figure..its distorted, also if possible use similar color patterns for all of the figures}}\label{fig:1}
\end{figure}

\subsection{Proposed Architecture}
\hl{``Proposed"?? may be refrain from using it...also...Section 3A is the subcomponent of the Architecture itself.--Subash }
Our architecture comprises two distinct phases. Initially, upon receiving a user query, we embark on the first phase where we extract common keywords between the query and our predefined keyword set. Subsequently, we assess the corresponding number of documents to be retrieved for each identified keyword. The average number of documents required across all relevant keywords is then computed. In the absence of any keywords in the query, we assign a small arbitrary number to accommodate all potential keywords. Once the number of documents to retrieve is determined, we proceed to retrieve the top-n documents, where 'n' represents the predefined set number. In the second phase, our Language Model (LLM), which could be any of several options such as Mistral or LLAMA2, processes the retrieved data and generates responses for the user. This process ensures the persistence of our Retrieval-Augmented Generation (RAG) system.
\newline
\newline
\newline
\begin{figure*}[h]
\centering
    \includegraphics[scale=0.50]{figs/BP_Achitechture.png}
    \caption{\AlgoName Architecture.\hl{rework on diagram, make it elegant-Subash}}\label{fig:2}
\end{figure*}

\subsection{Prospective Student Architecture}

\subash{If i am not wrong the current \AlgoName does not cater Prospective Student/Faculties etc...I mean we do not have seperate features like that...so I don't see value of including it here. }
For prospective students yet to decide on their academic majors, we've developed a set of questions aimed at discerning their departmental preferences. When a student responds to the initial question, their answer undergoes assessment by a lightweight Language Model (LLM) to determine if it constitutes a question. If affirmative, the query is passed to a larger LLM for processing and response generation using our local knowledge base. If the response does not constitute a question, the same LLM evaluates whether the statement provides insights into the student's interests or desired industry. Relevant insights are added to an information set. Once the required information is gathered, it's passed to the larger LLM for comprehensive processing, culminating in the recommendation of a department that: 

\begin{enumerate}
    \item exists within the university, and 
    \item aligns with the student's expressed interests{\newline}
\end{enumerate}

If the information set is incomplete, another question from the question set is presented, and the iterative process continues until the information set is deemed complete. This iterative approach ensures a thorough understanding of the student's preferences and aspirations, facilitating informed departmental recommendations. Conversely, for students who have already chosen a major, the system simplifies the process by directly inquiring about departmental interests. Once obtained, the user can freely query information related to that department. This architecture streamlines the decision-making process for undecided students and facilitates efficient information retrieval for those with predetermined majors.

\begin{figure}[h!]
\centering
    %\includegraphics[width=\linewidth,trim={0 0 1cm 0},clip]{figs/Prospective_Student_Arch.png}
    \includegraphics[scale=0.27]{figs/Prospective_Student_Arch.png}
    \caption{Architecture of prospective students who have not decided the majors.}\label{fig:2}
\end{figure}

%In this section we discuss three aspects of \AlgoName. First, we discuss the implementation details where we 
%This section is structured into three specific subsections. In \ref{implementation-detail}, we explain the technical process behind developing \AlgoName. Then we discuss key insights we gather concerning retrieval methods and 
%In section \ref{discussion}, we delve into the insights concerning various data retrieval methods andexplore their practical implications within the developed system. Furthermore, we discuss  %In \ref{limitations}, we explore the constraints and shortcomings encountered and provide our plan for the future.


\end{comment}


%\subsection{Overall Evaluation Criteria}

%\hl{remove this subsection-Subash}

% \hl{to evaluate the performance of our system we conduct a 2 pronged approach including qualitative and quantative. For quantative....RAGAS, for Qualitative... SUS. In the following subsection we first explain the dataset and then explain these approach in greater details.  }

% \subsection{Evaluation Metrics}

% In order to thoroughly assess the accuracy and effectiveness of our ground truths, we employ a rigorous framework known as Retrieval Augmented Generation Assessment (RAGAS) \cite{jeong2023generative} \cite{zhang2023mitigating}. This framework evaluates three key aspects of our RAG pipeline: ground truth labels (including context recall and answer correctness), automatic test data generation, and component-specific evaluations of the RAG pipeline, such as the retriever component and the generator component \cite{mahboub2024evaluation}. For the retriever component, we measure context precision and context recall. For the generator component, we assess faithfulness and answer relevancy \cite{chen2024benchmarking}. 


% \subash{abrupt starting of the section? may be provide some transition sentence before the beginning of the paragraph...} We have defined ground truths across eight engineering departments, each with questions and their corresponding answers, as detailed in the Appendix~\ref{app:ground_truths}.To assess these ground truths, we have employed a Retrieval-Augmented Generation Assessment (RAGAS) \cite{jeong2023generative} \cite{zhang2023mitigating}. This framework evaluates three key aspects of our ground truths: ground truth labels (including context recall and answer correctness), automatic test data generation, and component-specific evaluations of the RAG pipeline, such as the retriever component and the generator component \cite{mahboub2024evaluation}. For the retriever component, we measure context precision and context recall. For the generator component, we assess faithfulness and answer relevancy \cite{chen2024benchmarking}. 



% \hl{Such and such}



% \subash{Move Preprocessing  content from architecture section here and have a new subsection ``Data"}

% \subash{I don't see mention of RAGAS score at all? [0-1] 1 being optimal? Also, remove equations/ formula to calculate these metrics. the combination for these metrics should give you a RAGAS score...which is your final Score..For end-to-end evaluation we only need ``semantic similarity" and ``answer correctness'' } 
% \hl{also, justify why we use RAGAS out of others???, Why not BLUE, ROGUE, Perplexity??...This should be fairly easy to integrate.}


% \subsubsection{Context Precision}
% Context Precision assesses whether the defined ground truths include relevant items in the context, particularly those with a higher rank. It is calculated as follows:
% \begin{equation}
% \begin{split}
% \text{Context Precision@k} = \frac{\sum \text{precision@k}}{\text{total number of relevant items}}
% \end{split}
% \label{eq:context_precision}
% \end{equation}

% \begin{equation}
% \text{Precision@k} = \frac{\text{true positives@k}}{\text{true positives@k} + \text{false positives@k}}
% \label{eq:precision_k}
% \end{equation}
% Where K is the total number of chunks in the contexts.

% \subsubsection{Context Recall}
% Context recall evaluates how well the retrieved context matches the annotated answer, which serves as the ground truth. This metric is calculated as follows:
% \begin{equation}
% \text{context recall} = \frac{\text{GT sentences that can be attributed to context}}{\text{Number of sentences in GT}}
% \label{eq:context_recall}
% \end{equation}

% \subsubsection{Faithfulness}
% This metric assesses the factual accuracy of the generated answer. It is expressed with the following equation:


% \begin{equation}
% \text{Faithfulness score} = \frac{\text{Number of inferred claims}}{\text{Total number of claims}}
% \label{eq:faithfulness_score}
% \end{equation}

% \subsection{Accuracy and Reliability of Responses}

% This section is divided into three parts: Data-Driven Analysis, Comparative Analysis of Retrieval Efficiency, and Qualitative Assessment. In the Data-Driven Analysis \ref{app: data-driven}, we explore the assessment and evaluation using the RAGAS framework, including interactive visualization. The Comparative Analysis of Retrieval Efficiency \ref{app: retrieval-efficiency} delves into various retrievals' performance on top of our ground truths. Lastly, the Qualitative Assessment \ref{app: qualitative-assessment} discusses the \AlgoName interaction with the system usability scale and emphasizes its performance.


%In particular, we Splitting and Chunking text effectively is important to get best performance from RAG chatbot systems. By splitting text effectively, RAG models can generate a more accurate response that is contextually appropriate. We opted for \emph{recursive chunking} and utilize \emph{RecursiveCharacterTextSplitter} available through LangChain with chunk size of \hl{1500} and overlap of \hl{300} to split JSON file.Initially, we employed a recursive text splitter to divide research papers into smaller, more manageable sections. The segmentation approach was determined by characteristics such as the size of each section and the amount of overlap between them. Subsequently, we transformed the textual data into vectorized representations utilizing an embedding model, which could be chosen from pre-existing alternatives or tailored to suit our particular requirements. The data in vectorized form was subsequently saved on a local storage device. Through the process of integrating our well-organized data into a unified database, the efficiency of our model's operations significantly improved. For example, instead of searching through separate databases for each department, it could find what it needed in one place, speeding up our responses and saving time. Moreover, by eliminating noise and inconsistencies, the large language model (LLM) could better understand and utilize the information available, resulting in higher-quality outputs.


% \begin{figure*}[ht!]
% \centering
% \includegraphics[width=0.6\textwidth, height=0.35\textheight]{fixed_heatmap_retrieval_method_performance.png} 

% \caption{Comparative heatmap of retrieval methods by precision, recall, faithfulness, and relevancy across question categories.}
% \label{fig:heatmap_plot_overall}
% \end{figure*}


% \subash{Add a small subsection ``Implementation Detail and Discussion" and describe hw/sw/technology used during the development}
% This section is organized to facilitate readers' understanding of the technology driving the development of \AlgoName and to outline the recognized gaps, challenges, and limitations we faced during the development of LLM-based chatbot within educational environments.

% \subash{remove Overall Assessment}

% \subsubsection{Overall Assessment}

% \hl{need to discuss waht to write in this section....Subash}

% \hl{Upon evaluating two different types of retrievers within our \AlgoName system, namely an Ensemble Retriever and one based on the Chroma Database, several observations emerged. Firstly, regarding the ensemble retriever, which is recognized for its hybrid nature due to its strong performance across various downstream tasks, our initial expectation was for it to generate highly comprehensive and contextualized responses. However, we noticed a discrepancy in the actual responses received. Our investigation revealed that this approach does not fully utilize the maximum token thresholds (16k) during response generation, leading to less contextualized outputs. Despite retrieving documents based on varying K values, attempts to enhance document size and alter questioning methods within \AlgoName did not yield the desired effect. Ultimately, it was found that increasing the value of K did not leverage the maximum token thresholds for response generation.

% On the other hand, the retriever based on the Chroma Database yielded satisfactory results. It employs three search approaches: cosine search, similarity threshold search, and maximum marginal relevancy (MMR). These methods utilize a number of K and a similarity threshold value to determine document relevance based on user queries. Among these approaches, the similarity threshold search demonstrated satisfactory performance. We conducted similar test cases as with the ensemble retriever, such as altering question themes and adjusting K values and similarity thresholds. Moreover, our testing revealed that this retriever performs best when allowed to utilize the entire 16,000 token limit. This suggests that the retriever leverages the full context provided to deliver the optimal result. In addition to these, an important finding was that increasing the number of thresholds resulted in faster responses but also produced irrelevant outputs. Nonetheless, optimizing K and similarity threshold values is essential to achieve the desired outcomes with this retriever} \subash{This needs an update--Discuss this tomorrow in the meeting.}.



% Upon evaluating the comprehensive effectiveness of our methodology, it becomes apparent that the process of transitioning from data acquisition to retrieval strategy was not devoid of obstacles and required iterative improvements. Our methodology comprised multiple critical phases, each customized to enhance the acquisition and application of data from an extensive variety of sources within the ecosystem of Mississippi State University (MSU). 

% Initially, our approach prioritized unbiased and thorough data collection, employing one crawler to collect a total of 42 data from every single department at MSU. The segmentation insights contained in the resulting JSON files \cite{moller2021empirical} serve as the fundamental basis for subsequent analysis and retrieval. However, to prevent unwanted Unicode characters \cite{bettels1993unicode} and ensure data integrity, a denoising method \cite{yu2019deep} was required due to the sheer volume and diversity of the data. The process of generating embeddings \cite{keraghel2024beyond} from these segments represented a critical milestone in our methodology, as it enabled the conversion of unprocessed textual data into a format that could be easily retrieved and analyzed. The "RecursiveCharacterTextSplitter" \cite{lin2024revolutionizing} was utilized with selected parameters to produce embeddings that held significance. Furthermore, the OpenAI Embedding model "text-embedding-3-large" \cite{harris2024enhancing} \cite{xian2024vector} \cite{goel2024using} was selected to emphasize our commitment to utilizing cutting-edge tools for maximum efficiency.

% Importantly, our priority to utilize Chroma DB \cite{xie2023brief} for storing embeddings as a vector store retriever was based on thorough experimentation and comparative assessment. Opting for the Similarity Score Threshold search method \cite{assfalg2006similarity}, set at a threshold of 0.2, proved to be the most efficient approach for retrieving documents that demonstrated both relevance and diversity. This method not only sidestepped the limitations posed by token constraints but also generated reliable responses across a wide range of queries.

% The thorough evaluation of retrieval techniques, especially the Ensemble method \cite{zhang2024arl2}, offered valuable perspectives on the advantages and drawbacks of different approaches. Contrary to initial assumptions, combining BM25Retriever \cite{gangadhar2023retrieval} and Chroma DB in the Ensemble model did not achieve results comparable to those of the Singular Similarity Score Threshold approach. This highlights the intricate relationship between retrieval algorithms and the varied characteristics of the analyzed data.

% Our comprehensive evaluation demonstrates a rigorous methodology and subsequent iterative improvement. Through the implementation of state-of-the-art technologies and the adoption of a data-centric methodology, we have made every effort to optimize the scope and quality of insights extracted from the departmental environment at MSU. Nevertheless, as we navigate the constantly evolving landscape of information retrieval and analysis, it remains imperative that we persist in refining and enhancing our methodology.


%which not only made it publicly accessible but also showcased the robustness and effectiveness of our Python-based development in improving \AlgoName for educational purposes.


% To enhance BarkPlug's functionality and widen its usability, we are planning several key upgrades. These include adding support for multiple languages to cater to a diverse user base, integrating ASR and text conversion features to enable various interaction modes, and improving the retrieval algorithms to boost the accuracy and relevance of the information provided.  Moreover, we aim to apply the map-reduced document chain approach from LangChain to overcome the OpenAI API’s token limitations. Through these improvements, we aim to transform BarkPlug into a more reliable and accessible educational tool across varied settings.

% While recent studies shed light on the potential educational uses of chatbot technology, they also reveal persistent challenges. Despite their ability to offer immediate support and tailored learning experiences, these tools are hindered by issues like out-of-vocabulary issues \cite{huang2023let}, inconsistent content relevance \cite{huang2023survey}, and the need for frequent updates \cite{feng2023knowledge}. Moreover, the integration of large language models like ChatGPT introduces new complexities such as transparency \cite{graf2023chatgpt}, accountability \cite{wu2022ai}, and ethical concerns in academic contexts \cite{wu2024new}.

% These challenges underscore the necessity for further research and development of chatbot integration strategies in educational settings. Overcoming technical obstacles is crucial \cite{chang2024survey}, but so is navigating educational and ethical considerations. Through comprehensive research efforts, developers and educators can collaborate to explore methods for maximizing chatbot effectiveness while mitigating potential drawbacks. Ultimately, the aim is to fully utilize chatbot technology's potential in classrooms to enhance academic achievement and student learning.


